Multi-Temporal Relationship Inference in Urban Areas

Finding multiple temporal relationships among locations can benefit a bunch of urban applications, such as dynamic offline advertising and smart public transport planning. While some efforts have been made on finding static relationships among locations, little attention is focused on studying time-aware location relationships. Indeed, abundant location-based human activities are time-varying and the availability of these data enables a new paradigm for understanding the dynamic relationships in a period among connective locations. To this end, we propose to study a new problem, namely multi-Temporal relationship inference among locations (Trial for short), where the major challenge is how to integrate dynamic and geographical influence under the relationship sparsity constraint. Specifically, we propose a solution to Trial with a graph learning scheme, which includes a spatially evolving graph neural network (SEENet) with two collaborative components: spatially evolving graph convolution module (SEConv) and spatially evolving self-supervised learning strategy (SE-SSL). SEConv performs the intra-time aggregation and inter-time propagation to capture the multifaceted spatially evolving contexts from the view of location message passing. In addition, SE-SSL designs time-aware self-supervised learning tasks in a global-local manner with additional evolving constraint to enhance the location representation learning and further handle the relationship sparsity. Finally, experiments on four real-world datasets demonstrate the superiority of our method over several state-of-the-art approaches.

==> section/tbl-symbol.tex <==
\begin{table}[t]
	\mycaption{Mathematical notations.
	}
	\vspace{-3ex}
	\label{table-symbol}
	\begin{tabular}{cl}
		\toprule
		% \midrule
		% \midrule
		Notation	&	Description	\\
		\midrule
		% \midrule
		\proteinV,\ligandV	& The atom node sets of protein and ligand \\
		\proteinM,\ligandM	& The 3D position matrices of protein and ligand \\
		\graph	& The complex interaction graph	\\
		$a_i$	& The $i$-th atom node in \graph \\
		$e_{ij}$ & The directed edge from atom $a_i$ to atom $a_j$ \\
		$\mathcal{N}_{e}(a_i)$ & The neighboring edges of atom $a_i$ \\
		$\mathcal{N}_{e}(e_{ij})$ & The neighboring edges of edge $e_{ij}$ \\
		$\bm{a}_{i}$, $\bm{e}_{ij}$ & The embedding vectors of atom $a_i$ and edge $e_{ij}$  \\
		$\bm{d}_{ij}$ & The spatial embedding vector between $a_i$ and $a_j$ \\
        % \midrule
        % \midrule
        \bottomrule
        
	\end{tabular}
	\vspace{-3ex}
\end{table}


